Controller Datapath Aware Verification of Masked Hardware Generated via High Level Synthesis

Masking is a countermeasure against Power Side Channel Attacks (PSCAs) in both software and hardware implementations of cryptographic algorithms. Compared to software masking, implementing masked hardware is time consuming and error prone. Recent approaches, therefore, rely on High Level Synthesis (HLS) tools to automatically generate masked Register Transfer Level (RTL) hardware from verified masked software, significantly reducing design effort. Since HLS was never developed for security, HLS optimizations may impact PSCA security of the generated RTL. As a result, verifying the PSCA security of HLS generated masked RTL is crucial. Existing hardware masking verification tools can verify masked hardware, but may produce false positives when applied to HLS generated designs with controller datapath architectures obtained due to resource-shared datapath obtained via HLS. This work proposes a hardware masking verification strategy for HLS generated masked hardware. Our toolflow MaskedHLSVerif, performs state-wise formal verification of controller datapath RTL obtained via HLS, thereby avoiding false positives caused by resource-shared datapaths. Our tool flow correctly verifies standard cryptographic benchmarks, consisting of cascaded masked gadgets and the PRESENT S-box masked with gadgets, where existing tools like REBECCA reports false positives. The proposed tool-flow is able to detect masking flaws induced by HLS-optimizations as well.

==> defs.tex <==
\usepackage{xparse}
\newcommand{\bnm}{\begin{newmath}}
\newcommand{\enm}{\end{newmath}}

\newcommand{\bea}{\begin{eqnarray*}}%
\newcommand{\eea}{\end{eqnarray*}}%

\newcommand{\bne}{\begin{newequation}}
\newcommand{\ene}{\end{newequation}}

\newcommand{\bal}{\begin{newalign}}
\newcommand{\eal}{\end{newalign}}

\newenvironment{newalign}{\begin{align}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{align}}

\newenvironment{newmath}{\begin{displaymath}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{displaymath}}

\newenvironment{neweqnarrays}{\begin{eqnarray*}%
\setlength{\abovedisplayskip}{-4pt}%
\setlength{\belowdisplayskip}{-4pt}%
\setlength{\abovedisplayshortskip}{-4pt}%
\setlength{\belowdisplayshortskip}{-4pt}%
\setlength{\jot}{-0.4in} }{\end{eqnarray*}}

\newenvironment{newequation}{\begin{equation}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{equation}}


\newcounter{ctr}
\newcounter{savectr}
\newcounter{ectr}

\newenvironment{newitemize}{%
\begin{list}{\mbox{}\hspace{5pt}$\bullet$\hfill}{\labelwidth=15pt%
\labelsep=4pt \leftmargin=12pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{3pt} }}{\end{list}}


\newenvironment{newenum}{%
\begin{list}{{\rm (\arabic{ctr})}\hfill}{\usecounter{ctr} \labelwidth=17pt%
\labelsep=5pt \leftmargin=22pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{2pt} }}{\end{list}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Figure and table macros
%

\newcounter{mytable}
\def\mytable{\begin{centering}\refstepcounter{mytable}}
\def\endmytable{\end{centering}}

\def\mytablecaption#1{\vspace{2mm}
  \centerline{Table \arabic{mytable}.~{#1}}
  \vspace{6mm}
  \addcontentsline{lot}{table}{\protect\numberline{\arabic{mytable}}~{#1}}
}


\newcounter{myfig}
\def\myfig{\begin{centering}\refstepcounter{myfig}}
\def\endmyfig{\end{centering}}

\def\myfigcaption#1{
             \vspace{2mm}
             \centerline{\textsf{Figure \arabic{myfig}.~{#1}}}
             \vspace{6mm}
             \addcontentsline{lof}{figure}{\protect\numberline{\arabic{myfig}}~{#1}}}


\newlength{\saveparindent}
\setlength{\saveparindent}{\parindent}
\newlength{\saveparskip}
\setlength{\saveparskip}{\parskip}

\newcommand{\decOracle}{\textbf{Dec}}

\newcommand{\negsmidge}{{\hspace{-0.1ex}}}
\newcommand{\cdotsm}{\negsmidge\negsmidge\negsmidge\cdot\negsmidge\negsmidge\negsmidge}

\def\suchthatt{\: :\:}
\newcommand{\E}{{\rm I\kern-.3em E}}
\newcommand{\Prob}[1]{{\Pr\left[\,{#1}\,\right]}}
\newcommand{\Probb}[2]{{\Pr}_{#1}\left[\,{#2}\,\right]}
\newcommand{\CondProb}[2]{{\Pr}\left[\: #1\:\left|\right.\:#2\:\right]}
\newcommand{\CondProbb}[2]{\Pr[#1|#2]}
\newcommand{\ProbExp}[2]{{\Pr}\left[\: #1\:\suchthatt\:#2\:\right]}
\newcommand{\Ex}[1]{{\textnormal{E}\left[\,{#1}\,\right]}}
\newcommand{\Exx}{{\textnormal{E}}}
\newcommand{\given}{\ensuremath{\,\big|\,}}


\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}
\def\negl{\mathsf{negl}}


\newcommand{\secref}[1]{\mbox{Section~\ref{#1}}}
\newcommand{\appref}[1]{\mbox{Appendix~\ref{#1}}}
\newcommand{\thref}[1]{\mbox{Theorem~\ref{#1}}}
\newcommand{\defref}[1]{\mbox{Definition~\ref{#1}}}
\newcommand{\corref}[1]{\mbox{Corollary~\ref{#1}}}
\newcommand{\lemref}[1]{\mbox{Lemma~\ref{#1}}}
\newcommand{\clref}[1]{\mbox{Claim~\ref{#1}}}
\newcommand{\propref}[1]{\mbox{Proposition~\ref{#1}}}
\newcommand{\factref}[1]{\mbox{Fact~\ref{#1}}}
\newcommand{\remref}[1]{\mbox{Remark~\ref{#1}}}
\newcommand{\figref}[1]{\mbox{Figure~\ref{#1}}}
\renewcommand{\algref}[1]{\mbox{Algorithm~\ref{#1}}}
% \newcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
% Have to use \renewcommand because exists already in amsmath
\renewcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
\newcommand{\consref}[1]{\mbox{Construction~\ref{#1}}}
\newcommand{\tabref}[1]{\mbox{Table~\ref{#1}}}

\newcommand{\get}{{\:{\leftarrow}\:}}
\newcommand{\gett}[1]{\:{\leftarrow}_{#1}\:}
\newcommand{\getsr}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle\$$}}}\:}}
\newcommand{\getm}{{\:\leftarrow_{\mdist}\:}}
\newcommand{\getd}{{\:\leftarrow_{\ddist}\:}}
%\newcommand{\getm}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle \mdist$}}}\:}}
\newcommand{\getk}{{\:\leftarrow_{\kdist}\:}}
%\newcommand{\getk}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle \kdist$}}}\:}}
\newcommand{\getp}{{\:\leftarrow_{p}\:}}



\newcommand{\gamesfontsize}{\small}
\newcommand{\fpage}[2]{\framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}}
\newcommand{\mpage}[2]{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}

\newcommand{\hpages}[3]{\begin{tabular}{cc}\begin{minipage}[t]{#1\textwidth} #2 \end{minipage} & \begin{minipage}[t]{#1\textwidth} #3 \end{minipage}\end{tabular}}

\newcommand{\hpagess}[4]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #3 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #4 \end{minipage}
        \end{tabular}
    }

\newcommand{\hpagesss}[6]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #4 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #5 \end{minipage}
        &
        \begin{minipage}[t]{#3\textwidth}\gamesfontsize #6 \end{minipage}
        \end{tabular}
    }

\newcommand{\hpagessss}[8]{
        \begin{tabular}{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #5 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #6 \end{minipage}
        &
        \begin{minipage}[t]{#3\textwidth}\gamesfontsize #7 \end{minipage}
        &
        \begin{minipage}[t]{#4\textwidth}\gamesfontsize #8 \end{minipage}
        \end{tabular}
    }


\newcommand{\hfpages}[3]{\hfpagess{#1}{#1}{#2}{#3}}
\newcommand{\hfpagess}[4]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #3 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
        \end{tabular}
    }
\newcommand{\hfpagesss}[6]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #5 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.1}\gamesfontsize #6 \end{minipage}}
        \end{tabular}
    }
\newcommand{\hfpagessss}[8]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #5 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #6 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.1}\gamesfontsize #7 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#4\textwidth}\setstretch{1.1}\gamesfontsize #8 \end{minipage}}
        \end{tabular}
    }

\newcommand{\vecw}{\mathbf{w}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\load}{L}
\newcommand{\coll}{\mathsf{Coll}}
\newcommand{\nocoll}{\overline{\mathsf{Coll}}}


\newcommand{\Img}{\textsf{Img}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Fonts and symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\funcfont{\textsf}
\newcommand\variablefont{\texttt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NEW COMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def \Perm {\funcfont{Perm}}
\def \calC {{\mathcal{C}}}
\def \calU {{\mathcal{U}}}
\renewcommand{\u}{\ensuremath{u}}
\newcommand{\unew}{\ensuremath{\tilde{u}}}

\newcommand{\calN}{\mathcal{N}}
\def \sspace {{\mathcal{S}}}
\def \strings {{\mathcal{S}}}
\def \slen {{s}}
\def \kspace {{\mathcal{K}}}
\def \kspacesize {{m}}
\def \mspacesize {{n}}
\def \kdict {D}
\def \dictsize {d}
\newcommand{\kdist}{p_k}
\newcommand{\mdist}{\ensuremath{{W}}}
\newcommand{\alldist}{\rho}
\newcommand{\pwdist}{\transgen}
\newcommand{\ddist}{\rho_{dec}}
\newcommand{\PWset}{{\mathcal{P}}}  % TODO: fix, same as \pwdist
\newcommand{\PWsetvec}{\vec{\mathcal{P}}}
\newcommand{\PWvec}{\vec{P}}
\newcommand{\domvec}{\vec{D}}
\newcommand{\humanornot}{\vec{h}}
\newcommand{\dom}{\textsf{dom}}
%\def \kdist {{\kappa}}
%\def \mdist {{\mu}}
%\def \ddist {{\delta}}
\def \pspace {{\mathcal{P}}}
\def \mpspace {{\mathcal{MP}}}
\def \cspace {{\mathcal{C}}}
\def \key {\kappa}
\def \msg {M}
\def \seed {S}
\def \ctxt {C}
\def \ctxtpart {C_2}
\newcommand{\genprime}{{\textsf{GenPrime}}}
\newcommand{\isprime}{{\textsf{IsPrime}}}
\newcommand{\LeastLesserPrime}{{\textsf{PrevPrime}}}
\newcommand{\pwset}{\mathcal{S}}
\newcommand{\DTE}{{\textsf{DTE}}}
\newcommand{\encode}{{\textsf{encode}}}
\newcommand{\decode}{{\textsf{decode}}}

\newcommand{\DTEsingle}{{\textsf{1PW-DTE}}}
\newcommand{\encodesingle}{{\textsf{1PW-encode}}}
\newcommand{\decodesingle}{{\textsf{1PW-decode}}}

\newcommand{\DTErss}{{\textsf{RSS-DTE}}}
\newcommand{\encoderss}{{\textsf{RSS-encode}}}
\newcommand{\decoderss}{{\textsf{RSS-decode}}}

\newcommand{\DTEindep}{{\textsf{MPW-DTE}}}
\newcommand{\encodeindep}{{\textsf{MPW-encode}}}
\newcommand{\decodeindep}{{\textsf{MPW-decode}}}


\newcommand{\DTEsub}{{\textsf{SG-DTE}}}
\newcommand{\encodesub}{{\textsf{SG-encode}}}
\newcommand{\decodesub}{{\textsf{SG-decode}}}
\newcommand{\decodekamf}{{\textsf{KAMF-decode}}}
\newcommand{\DTEis}{{\textsf{IS-DTE}}}
\newcommand{\encodeis}{{\textsf{is-encode}}}
\newcommand{\decodeis}{{\textsf{is-decode}}}
\newcommand{\DTErej}{{\textsf{REJ-DTE}}}
\newcommand{\encoderej}{{\textsf{rej-encode}}}
\newcommand{\decoderej}{{\textsf{rej-decode}}}
\newcommand{\DTErsarej}{{\textsf{RSA-REJ-DTE}}}
\newcommand{\encodeRSAREJ}{{\textsf{rsa-rej-encode}}}
\newcommand{\decodeRSAREJ}{{\textsf{rsa-rej-decode}}}
\newcommand{\DTErsainc}{{\textsf{RSA-INC-DTE}}}
\newcommand{\encodeRSAINC}{{\textsf{rsa-inc-encode}}}
\newcommand{\decodeRSAINC}{{\textsf{rsa-inc-decode}}}
\newcommand{\DTEunf}{{\textsf{UNF-DTE}}}
\newcommand{\DTEnunf}{{\textsf{NUNF-DTE}}}


%\newcommand{\encodeis}{{\textsf{encode}_{\textrm{is}}}}
%\newcommand{\decodeis}{{\textsf{decode}_{\textrm{is}}}}
\newcommand{\rep}{\textsf{rep}}
\newcommand{\isErr}{\epsilon_{\textnormal{is}}}
\newcommand{\incErr}{\epsilon_{\textnormal{inc}}}
\def \enc {{\textsf{E}}}
\def \dec {{\textsf{D}}}
\def \SEscheme {{\textsf{SE}}}
\def \HEscheme {{\textsf{HE}}}
\def \CTR {{\textsf{CTR}}}
\def \encHE {{\textsf{HEnc}}}
\def \HIDE {{\textsf{HiaL}}}
\def \encHIDE {{\textsf{HEnc}}}
\def \decHIDE {{\textsf{HDec}}}
\def \decHE {{\textsf{HDec}}}
\def \encHEt {{\textsf{HEnc2}}}
\def \decHEt {{\textsf{HDec2}}}

\newcommand{\myind}{\hspace*{1em}}
\newcommand{\thh}{^{\textit{th}}} % th
\newcommand{\concat}{\,\|\,}
\newcommand{\dotdot}{..}
\newcommand{\emptystr}{\varepsilon}

\newcommand{\round}{\textsf{round}}

\newcommand{\alphabar}{\overline{\alpha}}
\newcommand{\numbinsbar}{\overline{b}}
\newcommand{\numballs}{a}
\newcommand{\numbins}{b}

%\def \encHE {{\sf{enc}^{HE}}}
%\def \decHE {{\sf{dec}^{HE}}}
%\def \encHEt {{\sf{enc}^{HE2}}}
%\def \decHEt {{\sf{dec}^{HE2}}}
\def \idealHE {{\mathcal{HE}}}
\def \IEnc {{\mathbf{\rho}}}
\def \IDec {{\mathbf{\rho^{-1}}}}
\def \OEnc {{\mathbf{Enc}}}
\def \ODec {{\mathbf{Dec}}}
\newcommand{\SimuProc}{\mathbf{Sim}}
\newcommand{\ROProc}{\mathbf{RO}}
\newcommand{\PrimProc}{\mathbf{Prim}}
\def \stm {g}
\def \istm {\hat{g}}
\def \kts {{f}}
\def \lex {{\sf lex}}
\def \part {part}
\def \kd {{\sf{kd}}}
\def \msgdist {{d}}
\def \keydist {{r}}
\def \ind {{\sf{index}}}
\def \kprf {z}
\def \adv {{\mathcal A}}
\def \pwds {u}
\newcommand{\mpw}{mpw}
\newcommand{\pw}{w}
\newcommand{\pwvec}{\vec{\pw}}
\newcommand{\vecx}{\vec{x}}
\def \tokens {v}
\def \calP{{\mathcal{P}}}
\def \template{{\mathcal{T}}}
\def \vaultset{{\mathcal{V}}}
\def \ext {{\sf ext}}
\def \offset {\delta}
\def \maxweight {\epsilon}
\def \advo {{\mathcal{A}}^{*}}

\newcommand{\Chall}{\textsf{Ch}}
\newcommand{\Test}{\textnormal{\textsf{Test}}}
\newcommand{\RoR}{\textsf{RoR}}
\newcommand{\MI}{\textnormal{MI}}
\providecommand{\MR}{\textnormal{MR}}
\newcommand{\MRCCA}{\textnormal{MR-CCA}}
\newcommand{\SAMP}{\textnormal{SAMP}}
\newcommand{\DTEgame}{\textnormal{SAMP}}
\newcommand{\KR}{\textnormal{KR}}
\newcommand{\advA}{{\mathcal{A}}}
\newcommand{\advR}{{\mathcal{R}}}
\newcommand{\advB}{{\mathcal{B}}} % 
\newcommand{\advC}{{\mathcal{C}}} % C
\newcommand{\advD}{{\mathcal{D}}} % D
\newcommand{\advE}{{\mathcal{E}}}
\newcommand{\advF}{{\mathcal{F}}}
\newcommand{\advG}{{\mathcal{G}}}
\newcommand{\advI}{{\mathcal{I}}}
\newcommand{\nextval}{\;;\;}
\newcommand{\TabC}{\texttt{C}}
\newcommand{\TabR}{\texttt{R}}
\newcommand{\Hash}{H}
\newcommand{\Cipher}{\pi}
\newcommand{\CipherInv}{\pi^{-1}}
\newcommand{\simu}{{\mathcal S}}
\newcommand{\prim}{P}
\newcommand{\maxguess}{\gamma}


\newcommand{\bigO}{\mathcal{O}}
\newcommand{\calG}{{\mathcal{G}}}

\def\sqed{{\hspace{5pt}\rule[-1pt]{3pt}{9pt}}}
\def\qedsym{\hspace{2pt}\rule[-1pt]{3pt}{9pt}}

\newcommand{\Colon}{{\::\;}}
\newcommand{\good}{\textsf{Good}}

\newcommand\Tvsp{\rule{0pt}{2.6ex}}
\newcommand\Bvsp{\rule[-1.2ex]{0pt}{0pt}}
\newcommand{\TabPad}{\hspace*{5pt}}
\newcommand\TabSep{@{\hspace{5pt}}|@{\hspace{5pt}}}
\newcommand\TabSepLeft{|@{\hspace{5pt}}}
\newcommand\TabSepRight{@{\hspace{5pt}}|}


\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\comma}{\textnormal{,}}

\renewcommand{\paragraph}[1]{\vspace*{6pt}\noindent\textbf{#1}\;}

\newcommand{\weirvault}{\textsf{Pastebin}\xspace}
\newcommand{\ndssvault}{\textsf{DBCBW}\xspace}




\newcommand{\reminder}[1]{ [[[ \marginpar{\mbox{$<==$}} #1 ]]] }

%
% New theorem types: (Already in CCS template)
%
\newtheorem{observation}{Observation}
%\newtheorem{definition}{Definition}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{fact}{Fact}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{corollary}{Corollary}[section]
% \newtheorem{proposition}{Proposition}
% \newtheorem{example}{Example}

%
% Definitions:
%
\def \blackslug{\hbox{\hskip 1pt \vrule width 4pt height 8pt
    depth 1.5pt \hskip 1pt}}
\def \qed{\quad\blackslug\lower 8.5pt\null\par}
% In-line QED, for ending a proof with a $$ formula
% In-line QED, for ending a proof with a $$ formula
\def \inQED{\quad\quad\blackslug}
\def \Qed{\QED}
\def \QUAD{$\Box$}
\def \Proof{\par\noindent{\bf Proof:~}}
\def \proof{\Proof}
\def \poly {\mbox{$\mathsf{poly}$}}
\def \binary {\mbox{$\mathsf{binary}$}}
\def \ones {\mbox{$\mathsf{ones}$}}
\def \rank {\mbox{$\mathsf{rank}$}}
\def \bits {\mbox{$\mathsf{bits}$}}
\def \factorial {\mbox{$\mathsf{factorial}$}}
\def \fr {\mbox{$\mathsf{fr}$}}
\def \pr {\mbox{$\mathsf{pr}$}}
\def \zon {\{0,1\}^n}
\def \zo  {\{0,1\}}
\def \zok {\{0,1\}^k}
\def \mo {s}


\def\utilcnt{\ensuremath{\mu_{\mathrm{cnt}}}}
\def\utiltime{\ensuremath{\mu_{\mathrm{time}}}}
\def\ex{\ensuremath{{\mathrm{ex}}}}
\def\rlx{\ensuremath{{\mathrm{rlx}}}}
\def\tp{\textsf{TP}}
\def\cp{\textnormal{\textsf{CP}}\xspace}
\def\edistcutoff{\edist}
\def\entcutoff{\ensuremath{m}}
\def\relentcutoff{{\sigma}}
\def\mutt{\mu_{\mathrm{tt}}}

\newcommand{\Hdot}{H(\mbox{ } \cdot \mbox{ }  , \mbox{ } \del)}


\newcounter{mynote}[section]
\newcommand{\notecolor}{blue}
\newcommand{\thenote}{\thesection.\arabic{mynote}}
\newcommand{\tnote}[1]{\refstepcounter{mynote}{\bf \textcolor{\notecolor}{$\ll$TomR~\thenote: {\sf #1}$\gg$}}}

\newcommand{\fixme}[1]{{\textcolor{red}{[FIXME: #1]}}}
\newcommand{\todo}[1]{{\textcolor{red}{[TODO: #1]}}}


\newcommand\ignore[1]{}


\newcommand\simplescheme{simple}


\newcommand{\KDF}{\mathsf{KDF}}
\newcommand{\salt}{\mathsf{sa}}
\newcommand{\PRF}{F}
\newcommand{\subgram}{\mathsf{SG}}
\newcommand{\popdomains}{\mathcal{D}}

\newcommand{\retrieve}{\textsf{Sync}}
\newcommand{\update}{\textsf{Insert}}

\newcommand{\dictW}{\textbf{D1}\xspace}
\newcommand{\dictF}{\textbf{D2}\xspace}

\newcommand{\str}{\text{str}}
\newcommand{\calS}{{\mathcal S}}

% \newcommand{\new}[1]{\textcolor{red}{\sf #1}}
\newcommand{\new}[1]{#1}


%% ------------------------- Rahul -----------------------
\newcounter{rcnote}[section]
\newcommand{\rcthenote}{\thesection.\arabic{rcnote}}
\newcommand{\rcnote}[1]{\refstepcounter{rcnote}{\bf \textcolor{magenta}{$\ll$RC~\rcthenote: {\sf #1}$\gg$}}}

\newcounter{mrnote}[section]
\newcommand{\mrthenote}{\thesection.\arabic{mrnote}}
\newcommand{\mrnote}[1]{\refstepcounter{mrnote}{\bf \textcolor{green}{$\ll$MR~\mrthenote: {\sf #1}$\gg$}}}

\newcounter{fknote}[section]
\newcommand{\fkthenote}{\thesection.\arabic{fknote}}
\newcommand{\fknote}[1]{\refstepcounter{fknote}{\bf \textcolor{blue}{$\ll$FK~\fkthenote: {\sf #1}$\gg$}}}

\newcounter{anote}[section]
\newcommand{\ajthenote}{\thesection.\arabic{anote}}
\newcommand{\anote}[1]{\refstepcounter{anote}{\bf \textcolor{cyan}{$\ll$AJ~\ajthenote: {\sf #1}$\gg$}}}



\newcommand{\mytab}{\hspace*{.4cm}}
\def\half{{1\over 2}}
\newcommand{\NT}[1]{\texttt{#1}}
\DeclareMathSymbol{\mlq}{\mathord}{operators}{``}
\DeclareMathSymbol{\mrq}{\mathord}{operators}{`'}
\newcommand{\calO}{{\mathcal O}}
\newcommand{\calA}{{\mathcal A}}
\newcommand{\kamfplus}{Kamouflage\textbf{+}\xspace}
% \newcommand{\genfrom}[1]{\;{\stackrel{\,#1}{\leftarrow}}\;}
\newcommand{\genfrom}[1]{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle#1$}}}\:}}
%\newcommand{\genfrom}[1]{\;\leftarrow{\tiny \$} #1\;}
\newcommand{\twopartdef}[4]
{
  \left\{
    \begin{array}{ll}
      #1 & \mbox{if } #2 \\[4pt]
      #3 & #4
      \end{array}
      \right.
}
\newcommand{\threepartdef}[6]
{
  \left\{
    \begin{array}{lll}
      #1 & \mbox{if } #2 \\
      #3 & \mbox{if } #4 \\
      #5 & \mbox{if } #6
      \end{array}
      \right.
}

\newcommand{\gt}[1]{\gamma_{#1,\maxdist}}
\newcommand{\gmt}[2]{\gamma_{#1,#2}}
\def\nh{\ensuremath{N}}
\def\ball{\ensuremath{B}}
\def\anh{\ensuremath{\tilde{N}_k}}
% \newcommand{\nh}[2]{{N_{#1}(#2)}}

\newcommand{\ballsizet}[1]{{\beta_{#1,\maxdist}}}
\newcommand{\ballsize}[2]{{\beta_{#1,#2}}}
\newcommand{\rh}[2]{{\bf R}_{#1, #2}}
\newcommand{\rhf}[2]{R_{f, \gamma}}
\newcommand{\realm}{{m}}
% \newcommand{\inputm}{{\tilde{m}}}
\newcommand{\lmid}{\ell_{\realm, m'}}
\newcommand{\cipherlength}{n}
\renewcommand{\SS}{\textsf{SS}}
\newcommand{\Rec}{\textsf{Rec}\xspace}
\newcommand{\rec}{\textsf{rec}\xspace}
\newcommand{\Rep}{\textsf{Rep}\xspace}
\newcommand{\Gen}{\textsf{Gen}}
\newcommand{\dis}{\textsf{dis}}

\def\chk{\textnormal{\textsf{Chk}}\xspace}
\def\reg{\textnormal{\textsf{Reg}}\xspace}
\def\exchk{\textnormal{\textsf{ExChk}}\xspace}
\def\adpchk{\textnormal{\textsf{AdpChk}}\xspace}
\def\RKROR{\textnormal{MKROR}\xspace}
\def\SRKROR{\textnormal{SKROR}\xspace}
\def\ROR{\textnormal{ROR}\xspace}
\def\ROBUST{\textnormal{ROB}\xspace}
\def\OFFDIST{\textnormal{OFFDIST}\xspace}
\def\POFFDIST{\overline{\textnormal{OFFDIST}}\xspace}
\def\OFFGUESS{\textnormal{OFFGUESS}\xspace}
\def\ONGUESS{\overline{\textnormal{ONGUESS}}\xspace}
\def\ONATTACK{\textnormal{ONATTACK}\xspace}
\def\adp{\ensuremath{\Pi\xspace}}
\def\Check{\textnormal{\textsf{Checker}}}
\def\CheckPtxt{\textnormal{\textsf{PChecker}}}
\def\trans{\textnormal{\ensuremath{T}}}
\def\transgen{\textnormal{\ensuremath{\mathcal{T}}}}
\def\pke{\ensuremath{\mathcal{E}}}
\def\pkenc{\ensuremath{\pke^{\mathrm{enc}}}}
\def\pkdec{\ensuremath{\pke^{\mathrm{dec}}}}
\def\sH{\ensuremath\mathrm{H}^s}
\def\H{\ensuremath{\mathsf{H}}\xspace}
\def\T{\ensuremath{\mathsf{T}}\xspace}
\def\W{\ensuremath{\mathsf{W}}\xspace}
\def\F{\ensuremath{\mathsf{F}}\xspace}
\def\ret{\ensuremath{\mathrm{return}}\xspace}
\def\cs{\ensuremath{t}} % Cache Size
\def\waitlen{\ensuremath{\omega}\xspace} %waitlist size
\newcommand{\M}{{\mathcal{M}}}
\newcommand{\ent}{{\bf H}}
\newcommand{\Hfuzzy}{{\mathrm{H}}^{\rm fuzz}}
\newcommand{\Hminfuzzy}{{\mathrm{H}}^{{\rm{fuzz}}}_{t,\infty}}
\newcommand{\Hpfuzzy}{{\mathrm{H}}^{{\rm{pfuzz}}}}
\newcommand{\Hinf}{{\bf H}^{{\rm \min}}_{\infty}}
\newcommand{\Hminpfuzzy}{{\bf H}^{{\rm pfuzz}}_{t,\infty}}


\def\sa{{\sf sa}}
\def\err{{\varepsilon}}%^{(e)}}}
\newcommand{\dist}{\mathcmd{p}}
\newcommand{\distest}{\hat{\mathcmd{p}}}
\newcommand{\distvec}{\mathbf{\dist}}
\newcommand{\distvecest}{\hat{\mathbf{p}}}
\newcommand{\w}{{w}}
\newcommand{\wnew}{\tilde{w}}
\newcommand{\m}{{w}}
\newcommand{\mnew}{{\tilde{m}}}
\newcommand{\mspacevec}{\mathcmd{\mathbf{W}}}
\newcommand{\mvec}{\mathcmd{\mathbf{\m}}}
\newcommand{\mvecss}[1]{\mvec_1\ldots\mvec_{#1}}
\renewcommand{\mspace}{\mathcmd{W}}
\newcommand{\mspacebot}{{\mspace}_\bot}

\newcommand{\similar}{\mathrm{sim}}
\newcommand{\similarvec}{\mathrm{\mathbf{sim}}}

\def \mvecnew{{\tilde{\mvec}}}
\newcommand{\mvecnewss}[1]{\mvecnew_1\ldots\mvecnew_{#1}}

\DeclareDocumentCommand{\edist}{o o}{
  \ensuremath{
    \IfNoValueTF{#1}{{d}}{{\sf d}(#1,#2)}
  }
}

\newcommand{\utilinc}{\mu}
\newcommand{\secloss}{\Delta}
\newcommand{\seclossg}{\Delta^\textnormal{greedy}}
\newcommand{\seclosso}{\Delta}
%\newcommand{\maxlambda}{\lambda^*}
%\newcommand{\maxfuzzlambda}{\tilde{\lambda}^*}
\newcommand{\fuzzlambda}{\lambda^\textnormal{fuzzy}}
\newcommand{\greedylambda}{\lambda^\textnormal{greedy}}
\newcommand{\greedylambdaon}{\tilde{\lambda}^\mathrm{on}}
\newcommand{\greedylambdaoff}{\tilde{\lambda}^\mathrm{off}}
\newcommand{\seclosson}{\secloss^\mathrm{on}}
\newcommand{\seclossoff}{\secloss^\mathrm{off}}
\def \edit {\ensuremath{e}}
\newcommand\error{e}
\newcommand\tab[1][1cm]{\hspace*{#1}}

\newcommand{\mathcmd}[1]{\ensuremath{#1}\xspace} % to use a command both in math mode and non-math mode
\newcommand{\minentropy}[1]{\ensuremath{\operatorname{H_\infty}\olrk{#1}}}
\newcommand{\fuzzyminentropy}[1]{\ensuremath{\operatorname{H^{fuzz}_{\maxdist, \infty}}\olrk{#1}}}
\providecommand{\condminentropy}[2]{\ensuremath{\operatorname{\tilde{H}_\infty}\olrk{#1|#2}}}
\newcommand{\s}{\mathcmd{s}}
\newcommand{\typo}{\mathcmd{\tilde{\m}}}
\newcommand{\typoj}[1]{\ensuremath{(\typo_{#1}, j_{#1})}}
\newcommand\typojprime[1]{{(\typo_{#1}, j'_{#1})}}
\renewcommand\contrib[2]{\mathsf{cont}\left[{#1}/{#2}\right]}
\def\typovec{\ensuremath{\{\typo_i\}_{i=1}}}
\def\opttypovec{\ensuremath{\{\typo^*_i\}_{i=1}}}
\def\slotguess{\textsf{SlotGuess}}
\def\typodist{\ensuremath{\tau_\pw}}
\def\cachedtypodist{\ensuremath{{\tilde{\tau}}_{\pw}}}
\def\typodistest{\ensuremath{{\hat{\tau}}_{\pw}}}
\def\incache{T_\pw}
\newcommand{\fuzzylambda}{\ensuremath{\lambda^{\mathrm{fuzzy}}}}
%\newcommand{\errorprob}[2]{\mathcmd{\tau_{#1}({#2})}}
\newcommand{\errordist}{\mathcmd{\tau}}
\newcommand{\famdist}{\mathcmd{\mathcal{W}}}
\def\guessw{\ensuremath{W}}
\newcommand{\precdist}{W}
\newcommand{\entdef}{Z}
\newcommand{\PW}{\mathcmd{\mathcal{W}}}
\newcommand{\cachedom}{\mathcmd{\mathcal{S}}}
\newcommand{\supp}{\mbox{supp}}
\newcommand{\olrk}[1]{\ifx\nursymbol#1\else\!\!\mskip4.5mu plus 0.5mu\left(\mskip0.5mu plus0.5mu #1\mskip1.5mu plus0.5mu \right)\fi}

\newcommand{\errorprob}[1]{\mathcmd{\tau_{#1}}}
\newcommand{\errorpr}[2]{\mathcmd{\errorprob{#1}{(#2)}}}
\newcommand{\Expectation}{\mathop{\mathbb E}}
\newcommand{\hash}[2]{\mathcmd{F(#1, #2)}}
\newcommand{\hashj}[3]{\mathcmd{F_{#3}(#1, #2)}}
\newcommand{\rhh}{\mathcmd{y}}
\newcommand{\x}{\mathcmd{x}}
\newcommand{\range}{\mathcmd{R}}
\newcommand{\lmm}{\mathcmd{l_\w}}
\newcommand{\rmm}{\mathcmd{r_\w}}
\newcommand{\conflict}[2]{\mathcmd{C_{#1, #2}}}
\newcommand{\Probsub}[2]{{\Pr_{#1}\left[\,{#2}\,\right]}}
\newcommand{\Condprobsub}[3]{{\Pr}_{#1}\left[\: #2\:\left|\right.\:#3\:\right]}
\newcommand{\wmid}{l_{\w, \w^\prime}}
\newcommand{\realhash}{\mathcmd{z}}
\newcommand{\collhash}{\mathcmd{z^\prime}}
\newcommand{\floor}[1]{\left \lfloor #1 \right \rfloor }
\newcommand{\ceiling}[1]{\left \lceil #1 \right \rceil }
\newcommand{\interval}{I}
% \newcommand{\p}[2]{p_{#1}(#2)}
\newcommand{\ssketch}{\mathcmd{\mathsf{S}}}
\newcommand{\tsketch}{\mathcmd{\msgsettingsym\mathsf{S}}}
\newcommand{\trivsketch}{\mathcmd{\tsketch_{\emptystr}}}
\newcommand{\WREC}{\mathcmd{\pcnotionstyle{W\pcmathhyphen{}REC}}}
\newcommand{\AREC}{\mathcmd{\pcnotionstyle{A\pcmathhyphen{}REC}}}
\newcommand{\WUTIL}{\mathcmd{\pcnotionstyle{W\pcmathhyphen{}UTIL}}}
\newcommand{\AUTIL}{\mathcmd{\pcnotionstyle{A\pcmathhyphen{}UTIL}}}
\newcommand{\indexset}{I}
\newcommand{\topset}{Z_1^*}
\newcommand{\cachedist}{T}
\newcommand{\pwdis}{R}
\newcommand{\onbudget}{q}
\newcommand{\blacklist}{\textsf{B}}
\newcommand{\blacklistlen}{\alpha}
\newcommand{\plaintextstate}{\bar{\state}}
\newcommand{\typocutoff}{\delta}
\newcommand{\plfuprob}{\ensuremath{\nu}}

\def\ballweight{\ensuremath{e_{\tilde{\tau}}}}
\newcommand{\Adv}{\textnormal{\textsf{Adv}}}
\newcommand{\AdvOFFLINE}[1]{\Adv^{\footnotesize\textnormal{\textrm{offdist}}}_{\footnotesize #1}}
\newcommand{\AdvOFFLINEP}[1]{\Adv^{\overline{\footnotesize\textnormal{\textrm{{offdist}}}}}_{\footnotesize #1}}
\newcommand{\AdvOFFGUESS}[1]{\Adv^{\footnotesize\textnormal{\textrm{offguess}}}_{\footnotesize #1}}
\newcommand{\AdvONGUESS}[1]{\Adv^{{\footnotesize\textnormal{\textrm{onguess}}}}_{\footnotesize #1}}
\newcommand{\AdvONATTACK}[1]{\Adv^{\footnotesize\textnormal{\textrm{onattack}}}_{\footnotesize #1}}
\newcommand{\AdvRKROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{mk-ror}}}_{\footnotesize #1}}
\newcommand{\AdvSRKROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{sk-ror}}}_{\footnotesize #1}}
\newcommand{\AdvROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{ror}}}_{\footnotesize #1}}
\newcommand{\AdvROBUST}[1]{\Adv^{\footnotesize\textnormal{\textrm{rob}}}_{\footnotesize #1}}

\newcommand{\advantage}[3]{\pcnotionstyle{\Adv}^{#1}_{#2}(#3)}
\newcommand{\neighbourhood}[2]{N_{#1}({#2})}
\newcommand{\rhhdist}{Y}
\newcommand{\fullerhash}{z}
\newcommand{\errorball}[2]{{B}^{\errordist}_{#1}(#2)}
\newcommand{\f}{f}
\newcommand{\pwmaxlen}{\ell}
\newcommand{\indexi}{i}
\newcommand{\indexq}{q}
\newcommand{\indexx}{x}
\newcommand{\replace}{\textsf{replace}}
\newcommand{\vecca}{\vecc{a}}
\newcommand{\veccb}{\vecc{b}}
\newcommand{\veccv}{\vecc{v}}
\newcommand{\coins}{r}
\renewcommand{\state}{\ensuremath{\mathsf{s}}}
\newcommand{\win}{\mathsf{win}}
\newcommand{\Chk}{\textsf{Chk}}
\newcommand{\PChk}{\textsf{PChk}}
\newcommand{\indexh}{h}
\newcommand{\randomZ}{Z}
\newcommand{\Cache}{\textnormal{\textsf{Cache}}}
\newcommand{\WarmupCache}{\textnormal{\textsf{WarmupCache}}}
\newcommand{\CacheUpdate}{\textnormal{\textsf{CacheUpdt}}}
\newcommand{\CacheInit}{\textnormal{\textsf{CacheInit}}}
\newcommand{\cachestate}{\ensuremath{\mathtt{S}}\xspace}
\newcommand{\cachestatelen}{\ensuremath{\sigma}\xspace}
\newcommand{\CacheLRU}{\textnormal{\textsf{CacheLRU}}}
\newcommand{\CacheLRUUpdate}{\textnormal{\textsf{UpdateLRU}}}
\newcommand{\CacheLRUInit}{\textnormal{\textsf{InitLRU}}}


\newcommand{\zxcvbn}{\textnormal{\textsf{zxcvbn}}\xspace}
\newcommand{\bad}{\textnormal{\textsf{bad}}}
\newcommand{\wait}{z}
\newcommand{\PKE}{\textnormal{\textsf{PKE}}}
\newcommand{\pkegen}{\mathcal{K}}
\newcommand{\pkeenc}{\mathcal{E}}
\newcommand{\pkedec}{\mathcal{D}}
\newcommand{\pkectxtspace}{\mathcal{C}_{\pkeenc}}
\newcommand{\pk}{{pk}}
\newcommand{\sk}{{sk}}
\newcommand{\PBE}{\textnormal{\textsf{PBE}}}
\newcommand{\utility}{\textsf{Utility}}

\newcommand{\skegen}{\ensuremath{\mathsf{K}}}
\newcommand{\skeenc}{\ensuremath{\mathsf{E}}}
\newcommand{\skedec}{\ensuremath{\mathsf{D}}}
\newcommand{\skectxtspace}{\ensuremath{\mathcal{C}_{\skeenc}}}
\newcommand{\ske}{\textnormal{\textsf{SKE}}}
\newcommand{\SE}{\textnormal{\textsf{SE}}}
\newcommand{\sekg}{\mathcal{K}}
\newcommand{\seenc}{\mathcal{E}}
\newcommand{\sedec}{\mathcal{D}}
\newcommand{\saltlen}{{\ell_{\mathrm{salt}}}}

\newcommand{\skk}{\textnormal{\textsf{k}}}
\newcommand{\cipherske}{{c}}
\newcommand{\cipherpke}{{c}}
\newcommand{\SH}{\textnormal{\textsf{SH}}}
\newcommand{\FH}{\textnormal{\textsf{H}}}
\newcommand{\counter}{\textnormal{\textsf{Count}}}
\newcommand{\indexp}{p}
\newcommand{\ciphertextspace}{\mathcal{C}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\indexr}{r}
\newcommand{\vecc}[1]{\mathbf{#1}}
\newcommand{\sawait}{\overline{\sa}}
\newcommand{\skkwait}{\overline{\skk}}
\newcommand{\hwait}{\overline{\indexh}}
\newcommand{\randomY}{Y}
\newcommand{\indexm}{m}
\newcommand{\hashtable}[1]{H[#1]}
\newcommand{\SHlen}{k_1}
\newcommand{\FHlen}{k_2}
\newcommand{\valid}{\textnormal{\textsf{valid}}}
\newcommand{\skepsilon}{\epsilon_{ske}}
\newcommand{\pkepsilon}{\epsilon_{pke}}
\newcommand{\hybindex}{j}

\newcommand{\DL}{\textnormal{DL}}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\indicator}{\mathbb{I}}
\newcommand{\cipherspace}{\mathcal{C}}
\newcommand{\pkemsgspace}{\mathcal{M}_\pkeenc}

\newcommand{\pkecipher}{c}
\newcommand{\skecipher}{{c}}
\newcommand{\pkemsg}{m}
\newcommand{\skemsg}{{m}}
\newcommand{\skemsgspace}{ \msgspace_{\skeenc}}
\newcommand{\upperb}{\alpha}

\newcommand{\ffbox}[1]{
   \setlength{\fboxsep}{-1\fboxrule}
   \fbox{\hspace{1.2pt}\strut#1\hspace{1.2pt}}}


\newcommand{\statespace}{S}
\newcommand{\targuess}{\textsf{TarGuess}}
\newcommand{\untarguess}{\textsf{UnTarGuess}}

\newcommand{\accept}{\texttt{accept}}
\newcommand{\reject}{\texttt{reject}}
\newcommand{\threshold}{\ensuremath{\tau}}
\newcommand{\clfthreshold}{\ensuremath{\theta}}
\newcommand{\far}{\ensuremath{\alpha}}
\newcommand{\frr}{\ensuremath{\beta}}
\newcommand{\fpr}{\ensuremath{\nu}}
\newcommand{\fnr}{\ensuremath{\gamma}}
\newcommand{\FPR}{\textrm{FPR}}
\newcommand{\FNR}{\textrm{FNR}}


\newcommand{\matchalgo}{\mathcal{L}}
\newcommand{\matchalgovec}{\mathcal{\mathbf{L}}_\sslen}
\def \score {\theta}
\newcommand{\indexjvec}{\ensuremath{\mathcmd{\mathbf{j}}\xspace}}
\def\k{k}
\newcommand{\add}{\funcfont{Add}}
\newcommand{\accuracy}{\funcfont{Accuracy}}
\def\acc{\delta}
\def \MS {\funcfont{MS}}
\def \MRec {\funcfont{MRec}}
\newcommand \MSt{\MS^{\matchalgo}_\sslen}
\newcommand \MRect{\MRec^{\matchalgo}_\sslen}
\def \nmatches {\ensuremath{l}}
\def \D{D}
\def \Dmod{\tilde{D}}
\def \mlen{n}
\def \sslen{t}
\def \secret{s}
\def \secretvec{\mathbf{s}}
\newcommand{\sketch}{{\funcfont{sketch}}}
\newcommand{\sketchval}{v}
\def \recover{\funcfont{recover}}
\def \verify{\funcfont{verify}}
\def \q{q}
\def\fp{\alpha}
\def\fn{\beta}
\def\tp{\gamma}
\newcommand{\one}{\ensuremath{\mathbbm{1}}}
\newcommand{\seclen}{\ell}
\newcommand{\Overify}{{\mathcal{O}_\funcfont{vrfy}}}
\newcommand{\Omatch}{\mathcal{O}_\funcfont{match}}
\newcommand{\ith}[2]{#1_{#2}}
\newcommand{\jth}[2]{#1^{#2}}
\newcommand{\mspacei}{\ith{\mspace}{i}}
\newcommand{\errori}{\ith{\error}{i}}
\newcommand{\matchalgoi}{\ith{\matchalgo}{i}}
\newcommand{\mvecbar}{\overline{\mvec}}
\newcommand{\mvectilde}{\tilde{\mvec}}
\newcommand{\angbrac}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\clf}{\mathcal{C}}
\newcommand{\clft}{\clf_\sslen}
\newcommand{\clfest}{\mathcal{\hat{\clf}}}
\newcommand{\clfq}[1]{{\clf^q_{#1}}}
\newcommand{\nclf}{r}
\newcommand{\oclf}{\omega}
\newcommand{\biosketch}{\funcfont{TenSketch}\xspace}
\newcommand{\tensketch}{\funcfont{TenSketch}\xspace}

\newcommand{\hvec}{\mathbf{h}}
\newcommand{\insertr}{\mathsf{insert{\scriptstyle\$}}}
\newcommand{\dbmsg}{\ensuremath{\mathcal{F}}}
\newcommand{\dbmsgs}{\ensuremath{\{\dbmsg_i\}}}
\newcommand{\dbid}{\mathcal{I}}
\newcommand{\db}{\ensuremath{D}}
% \newcommand{\dbs}{\ensuremath(\dbid,\{\dbmsg_i\})}
\newcommand{\dbs}{\ensuremath(\dbid,\dbmsg)}
\newcommand{\dbsprime}{\ensuremath(\dbid',\dbmsg')}
\newcommand{\dbsize}{N}
\def \dblen{N}
\def\mhat{\hat{\mvec}}
\def\findmatches{\funcfont{\footnotesize FindMatches$^{\matchalgo}$}}
\newcommand{\setss}[1]{\SS^\Delta_{#1}}
\newcommand{\setrec}[1]{\Rec^\Delta_{#1}}
\newcommand{\setsst}{\setss{\sslen}}
\newcommand{\setrect}{\setrec{\sslen}}
\newcommand{\costs}{{c_s}}
\newcommand{\costc}{{c_c}}
\NewDocumentCommand{\indseq}{ O{1} O{r} }{{#1}\ldots {#2}}
\newcommand{\seq}[2]{{{#1}_1,\ldots,{#1}_{#2}}}
\newcommand{\relu}{\funcfont{ReLu}}
\newcommand{\fcrelu}[1]{\funcfont{FC}_{\relu}^{#1}}
\newcommand{\gencliq}{\funcfont{GenTupIncr}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> images/mainflow.tex <==
% \section{Diagrammatic view of Multisketch operations}\label{app:mainflow}  

% A user registers with a user id $\u$ and a vector of biometric templates
% $\mvec=\mvecss{\mlen}$. Multisketch uses two databases $\dbid$ and $\dbmsg$\@,
% where $\dbid$ contains user id $\u$ and the corresponding helper data
% $\sketchval$, and $\dbmsg$ contains the random permutation of the templates
% registered so far. Highlighted are the entries corresponding to a user $\u_4$
% with templates $\mvec_4=\mvec_{41}\ldots\mvec_{4\mlen}$.% and helper
%     % data $\sketchval_4$.
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
    >=stealth,
    node distance=2cm,
    database/.style={
      cylinder,
      cylinder uses custom fill,
      cylinder body fill=black!25!white,
      cylinder end fill=black!25!white,
      shape border rotate=90,
      aspect=0.25,
      minimum width=2em,
      minimum height=2em,
      draw
    },
    func/.style={
      rectangle,
      fill=red!25!white,
      minimum width=1cm,
      minimum height=1em,
      draw
    },
    cell/.style={
      rectangle,
      draw=black!50!white
    }
    ]
    \node (user) at (0, 0) {User};
    \node[func, right of=user, right=-1.1em, above=3em] (msketch) {$\MS$}; 
    \draw[below of=msketch, dashed, anchor=west] (.85,0.55) rectangle (5.9,-1.2); 
    \node[func, below of=msketch, anchor=east, below=1.95cm,fill=red!10!white,dashed] (mrecover) {$\MRec$};
    % \node[database, right of=user, anchor=south, above=1em, right=2cm] (db1) {$\dbid$};
    \matrix (db1) [right of=user, anchor=south, below=2pt, right=-0.1cm, 
    matrix of math nodes,
    column sep = -\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}}, 
    column 2/.style={nodes={cell}}, 
    anchor=west] {
      \u_1 & \sketchval_1\\
      \u_2 & \sketchval_2\\
      \u_3 & \sketchval_3\\
      |[draw,fill=blue!20]|\u_4 & |[draw,fill=blue!20]|\sketchval_4\\
    };
    \node[left of=db1, anchor=east,right=1.1cm] {$\dbid$};
    \matrix (db2) [right of=db1, left=25pt, matrix of math nodes,
    column sep = 2\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}},
    column 2/.style={nodes={cell}}, 
    column 3/.style={nodes={cell}}, 
    column 4/.style={nodes={cell}}, 
    column 5/.style={nodes={cell}}, 
    anchor=west] {
      \mvec_{21} &\mvec_{12} & |[draw,fill=blue!20]|\mvec_{43} &  & \mvec_{3\mlen} \\
      |[draw,fill=blue!20]|\mvec_{41} &\mvec_{32} & \mvec_{33} & |[draw=white]|\ldots & \mvec_{2\mlen} \\
      \mvec_{11} &|[draw,fill=blue!20]|\mvec_{42} & \mvec_{23} &  & \mvec_{1\mlen} \\
      \mvec_{31} &\mvec_{22} & \mvec_{13} & & |[draw,fill=blue!20]|\mvec_{4\mlen} \\
    };
    \node[left of=db2, left=-4pt] {$\dbmsg$};

    % \node[database,right of=db1] (db2) {$\dbmsg$};
    \node[func,below of=db1,anchor=north,above=8pt,left=8pt] (gu) {GetUser};
    \node[func,right of=gu,anchor=east,right=-5pt] (fm) {FindMatches};
    \node[func,below of=db1,anchor=east,below=2em,right=-3pt] (recover) {Recover};

    \draw[->,blue!50,thick] (user.north) |- node[black,near end,above]{$u, \mvec$} node[black,near end,below,font=\small]{register} 
    (msketch.west);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$u, \sketchval$} (db1);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$\mvec$} (db2);

    \draw[->,blue!50,thick] (user.south) |- ++(1,-0.9) node[black,near end,above]{$u, \mvectilde$} node[black,near end,below,font=\small]{login}   -| node[black,left,near end]{$u$}
    (gu.north);
    \draw[->,blue!50,thick] (user.south) |- ++(0,-0.9)  -- ++(3.1,0) |- node[black,near end, above]{$\mvectilde$}
    (fm.west);
    \draw[->,blue!50,thick] (db1.south) |- node[black,near end,above]{} (gu.east);
    \draw[->,blue!50,thick] (db2.south) |- node[black,near end,above]{} (fm.east);
    \draw[->,blue!50,thick] (gu.south) |- node[black,near end,above]{$\sketchval$} (recover.west);
    \draw[->,blue!50,thick] (fm.south) |- node[black,near end,above]{$\mvec'$} (recover.east);    
    \draw[->,blue!50,line width=2pt] (recover.south) -- node[black,near end,right]{$\mvec$ or $\bot$} ++(0, -0.65);
  \end{tikzpicture}
  % \rcnote{Rough sketch of the flow of the \biosketch.} 
  \caption{Diagram of multisketch as a part of an authentication service. 
  }
  \label{fig:mainflow}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/background_relatedwork.tex <==
\section{Background}
\label{sec:background}
In this section we give the background information on HLS for masked hardware generation, formal verification of masked hardware, and formal verification of masked hardware using REBECCA \cite{rebeccabloem2018formal}. 
\subsection{Using High-Level Synthesis to generate Masked Hardware Automatically}
\label{subsec:MaskedHLS}
Masking in software and hardware are different in that hardware masking needs to protect against the asynchronous behavior of computing hardware like glitches and transitions. A glitching input of a circuit can cause an intermediate wire to leak any combination of its secret inputs thus reducing the PSCA-security. In order to prevent these, masking schemes propose the usage of registers at strategic locations in the masked hardware such that glitches do not propagate to subsequently nullify masking security \cite{dom2016, HPC2020, comar}. Gadget-based masking schemes \cite{HPC2020} are a strategy of masking where an unmasked design made up of several affine (linear operations like boolean XOR, shift right or shift left) and non-affine (non-linear operations like boolean AND) can be modularly transformed to a masked designs, most often by replacing the non-affine operations with gadgets which are themselves masked. The composition of these gadgets into the hardware by their replacing the non-affine computations in a shared (masked) datapath results in a masked design due to the compositional properties of the gadgets. Several such masking gadgets exists such as the DOM, HPC1, HPC2, COMAR multiplication gadgets. Each of these gadgets have certain intermediate computations that needs to be registered when used for hardware masking in order to be un-effected by glitches. 

HLS has been used to generated masked hardware automatically from masked software due to the shortened design cycle and ease of use \cite{shortestpath2021}, \cite{hlsarx}, \cite{maskedhls}. HLS obtains a (often optimized) hardware design at RTL from a software specification via the following steps: scheduling, resource-allocation and binding, datapath and controller generation. For any arbitrary masking scheme, it is non-trivial to obtain a hardware masked design from a software masked design. However, for gadget-based masked designs, the process becomes simpler. To obtain a gadget-based masked hardware from a gadget-based masked software of the same algorithm, the following steps are performed: 
\begin{itemize}
    \item For each gadget in the gadget based masked software, identify the locations where registers need to be inserted according to the masking gadget specifications. These registers are mostly required in the masked hardware to arrest the propagation of glitches and maintain masking security in glitchy circuits \cite{glitch2005mangard, dom2016}. 
    \item Annotate these locations in a way that the HLS tool understands so that these computations results are stored in registers instead of wires in the output RTL.
    \item Paas this annotated software specification as input to the HLS tool to obtain the corresponding masked RTL design.
\end{itemize}

% \begin{itemize}
%     \item 
% \end{itemize}
% Hardware masking must ensure resilience against the asynchronous behavior of circuits such as those caused by \textit{glitches} that may cause the recombination of shares within the circuit, removing the masking security. Secondly, there are hardware masking verification tools \cite{HPC2020} to verify that a handwritten masked hardware design is secure. However, they are limited in applicability due to gaps in hardware masking verification theory \cite{moos2019glitch}, which prevents the scalability of verification to higher orders. Further, keeping in mind the development of new masking schemes/gadgets, there is an increased need for design-space exploration at the hardware level. Thus, developing secure masked hardware from scratch requires significant expertise in the design, verification, and design-space exploration of masked designs. 

% In contrast, software masking is easier to obtain from the algorithmic specification and easily verified \cite{compilerassistedmasking2012}. Therefore,  ways to obtain masked hardware from the corresponding masked software implementations would be beneficial. This is indeed a possibility, as the glitch-resistant hardware masking properties are a super-set of the software masking properties. Also, most glitch-resistant hardware-masked gadgets like DOM \cite{dom2016}, HPC1 and HPC2 \cite{pini2020}, and COMAR \cite{comar} have the same structure as their software-masked counterparts with additional registers to stop the propagation of glitches. Thus, in order to generate PSCA-secure masked hardware from masked software, a simple translation of intermediate code to RTL is desired. That can be followed by inserting registers at well-defined locations for state-of-the-art masking gadgets like DOM, HPC and COMAR. 

% In this regard, High-Level Synthesis (HLS), which automatically generates register transfer level (RTL) hardware from descriptions in C/C++, can be helpful. 
% A few recent works \cite{shortestpath2021} aim to utilize HLS to convert masked software implementations to masked hardware automatically. {\it In this work, we have shown that all stages of the HLS can hamper the security of masked circuits.}  

\subsection{Security Evaluation of Masked Hardware}
\label{subsec:formalVerificationofMasking}
There are two common approaches for evaluating the resistance of a masked design against PSCA:empirical leakage assessment and  formal verification.
    Empirical leakage assessment, which is done by statistical significance tests \cite{gilbert2011testing} to gauge the correlation between simulated (or real) power traces and the key, is a the most common approach. However, since these evaluations are practical they are not complete. On the other hand, formal verification tools can concretely state the PSCA-security of a masked implementation. The verification of software masking has advanced to a stage where they are very accurate and fast \cite{sleuth}. However, hardware masking verification tools are still unable to accurately determine the security of masked hardware implementations. This can be attributed to glitches at hardware that can disrupt the guarantee of masking security. State-of-the-art attacker models for masked hardware are yet unable to model such glitches and transitions accurately with scalability to higher orders. However, in contrast with empirical leakage assesment methods that are limited by the number of traces or the evaluated device, formal verification tools give provable security properties that the design satisfy or does not satisfy. Also, they provide information on the locality of the security vulnerability in the design.
\subsection{Formal Verification of Masked Hardware using REBECCA \cite{rebeccabloem2018formal}}
% \label{subsec:rebecca}
 
%     \subsubsection{REBECCA \cite{rebeccabloem2018formal}}
    \label{subsubsec:rebecca}
    REBECCA is a formal verification tool for verifying the masking security of hardware masked designs. 
    It takes as input a masked Verilog design, and a label file (.txt) that contains the labelling information of each input signal as a share, random, or public value. It also takes as input the masking security order (number of shares per sensitive input) for verification and the leakage model (with or without glitches indicated as static (S) and transient (T) respectively). It also internally generates a JSON configuration file using Yosys that has the gate wise information of the design under verification. Based on these inputs, REBECCA performs formal verification to assess whether the design is secure under the specified probing model \cite{isw, robustprobingmodel2018}. It generates a log file with which indicates if the cirucit is secure or not and if not then generates a counterexample trace that gives the location of the violation, helping the designer to debug the masking hardware. Using this flow REBECCA is able to verify all designs with a pipelined datapath based on a probing model \cite{isw, robustprobingmodel2018} and a security order $\ge 1$, albeit not so efficiently for higher orders.


    REBECCA performs the security verification starting at the inputs of the design by analyzing the labels at each gate's inputs and propagating them to their output using a set of rules derived from Fourier estimation. Each gate output is dependent on the gate inputs via a statistical dependency. REBECCA expresses a gate's output as function which is a sum of monomials over a the set of dependent inputs. Each coefficient in the monomial indicates the contribution of the set of inputs to the output of the gate. A non-zero coefficient corresponding to a input variable indicates a correlation between the function and the variable. Thus a coefficient approximately captures this dependency of a gate on a secret input and hence the calculation of these coefficients results in the estimation of the correlation of each gate to the sensitive inputs. If a correlation function contains non-zero coefficients corresponding to secret inputs and no correlation to uniformly masking variables, then there is a leak. This makes the calculation of leakages easy as only tracking whether the coefficients are $0$ results in the estimation of the security instead of a full Fourier Transform. 
REBECCA relies on the ISW probing model \cite{isw} with glitches in order to determine the security level of each gate from the Fourier coefficients. 
\textcolor{red}{do we need this subsection...?}
\subsubsection{Fourier Expansion of Boolean Functions}
% If \( S \triangle T = (S \setminus T) \cup (T \setminus S) \) denotes the symmetric difference of two sets \( S \) and \( T \), which REBECCA defines as the pointwise set difference of all elements. We write \( B = \{\text{true}, \text{false}\} \) for the set of Booleans. For a set \( X \) of Boolean variables, we identify an assignment \( f : X \to B \) with the set of variables \( x \) for which \( f(x) = \text{true} \). For a Boolean function \( f(X, Y) \) and an assignment \( x \subseteq X \), we write \( f|_x \) to denote the function \( f|_x(y) = f(x, y) \).

% {Fourier Expansion of Boolean Functions}

Below we borrow the definition of Fourier expansion as given in REBECCA \cite{rebeccabloem2018formal}:

% \begin{definition}[Statistical Independence]
% Let \( X \), \( Y \), and \( Z \) be sets of Boolean variables and let \( f : 2^X \times 2^Y \to 2^Z \). We say that \( f \) is statistically independent of \( X \) if for all \( z \) there is a constant \( c \) such that for all \( x \) we have \( | \{ y \mid f(x, y) = z \} | = c \).
% \end{definition}

% \begin{lemma}
% Let \( F : B^X \times B^Y \to B^Z \). Function \( F \) is statistically independent of \( X \) if and only if for all functions \( f : B^Z \to B \) we have that \( f \circ F \) is statistically independent of \( X \). 
% \end{lemma}
% \textit{Proof:} See Appendix A.

% To define Fourier expansions, we follow the exposition of \cite{ref32} and associate true with \(-1\) and false with \(1\). We can then represent a Boolean function as a multilinear polynomial over the rationals.

\textbf{Fourier Expansion}
Any Boolean function \( f: \{-1, 1\}^n \to \{-1, 1\} \) can be written in terms of monomials of its input variables \( x_1, x_2, \ldots, x_n \). Each monomial corresponds to a subset \( T \subseteq [n] \) where $n$ are the input indices. A monomial $\chi_T(X)$, $X = (x_1, x_2, \ldots, x_n)$ is defined as:
\[
\chi_T(X) = \prod_{i \in T} x_i.
\]

Thus, the function can be written as:
\[
f(X) = \sum_{T \subseteq [n]} \hat{f}(T) \chi_T(X),
\]
where \( \hat{f}(T) \) is the \emph{Fourier coefficient} for the subset \( T \), given by:
\[
\hat{f}(T) = \frac{1}{2^n} \sum_{X \in \{-1, 1\}^n} f(X) \cdot \chi_T(X).
\]

% The set of all such characters forms an orthonormal basis for the space of functions \( f: \{-1, 1\}^n \to \mathbb{R} \).

% \textbf{Note:} To distinguish arithmetic from Boolean operations, we use \( \cdot \) and \( + \) for multiplication and addition, and \( \wedge \), \( \oplus \) for Boolean AND and XOR, respectively.


\textbf{Example}

For the Boolean AND function: \( f(x, y) = x \wedge y \). Its Fourier expansion is:
\[
f(x, y) = \frac{1}{2} + \frac{1}{2}x + \frac{1}{2}y - \frac{1}{2}xy.
\]

For instance, if \( x = 1 \) (false), \( y = -1 \) (true), then:
\[
f(1, -1) = \frac{1}{2} + \frac{1}{2} - \frac{1}{2} + \frac{1}{2} = 1,
\]
which corresponds to ``false'' as expected for the Boolean AND operation.

% \subsection*{Key Points}
% \begin{enumerate}
%     \item The Fourier expansion uses monomials like \( x \cdot y \), which represent XOR in the \(\{-1, 1\}\) domain.
%     \item For any Boolean function \( f \), we have \( f^2 = 1 \).
%     \item The only linear two-variable functions are XOR: \( f = x \cdot y \) and XNOR: \( f = -x \cdot y \). All other Boolean functions are nonlinear and have all four Fourier coefficients non-zero: \( \hat{f}(\emptyset) \), \( \hat{f}(\{x\}) \), \( \hat{f}(\{y\}) \), and \( \hat{f}(\{x, y\}) \).
%     \item Fourier coefficients also encode statistical dependencies. For instance, the AND function has:
%     \begin{itemize}
%         \item A constant bias (non-zero \( \hat{f}(\emptyset) \)),
%         \item Positive correlation with each of \( x \) and \( y \),
%         \item Negative correlation with \( x \oplus y \).
%     \end{itemize}
% \end{enumerate}

There is a close connection between statistical dependence and the Fourier expansion of Boolean functions. REBECCA relies on an elementary result \cite{xiao1988spectral} which states that 
\textbf{Lemma}
A Boolean function \( f : \{ -1, 1 \}^n \to \{ -1, 1 \} \) is statistically independent of a set of variables \( X' \subseteq X \) if and only if for all \( T \subseteq X' \) it holds that \( \hat{f}(T) = 0 \) whenever \( T \neq \emptyset \).

\textcolor{red}{Till here...}

Let an ordered set \( X = \{x_0, \ldots, x_n\} \) denote the set of input variables. REBECCA partitions the input variables into three categories:
\begin{itemize}
    \item \( S = \{s_1, \ldots, s_j\} \) sensitive inputs that an attacker should not be able to recover via a statistical correlation to the output of any intermediate computation. 
    \item \( M = \{m_1, \ldots, m_k\} \) are masks that are uniformly independent random values that have no correlation to any secret and hence are used to de-correlate a secret input from intermediate computation results. 
    \item \( P = \{p_1, \ldots, p_l\} \) are all other known variables that can be known to the attacker without compromising the security of the algorithm.
    \end{itemize}

As an example let us consider the circuit in Figure \ref{fig:label_propagation}a. Table \ref{tab:rules}, denote the set of rules used by REBECCA to obtain the monomials with non-zero coefficients of a gate (labels) from the its inputs. Specifically, given the circuit in Figure \ref{fig:label_propagation}a, the inputs are labelled as shown in Table \ref{tab:example} where $s_m$ denotes a secret masked with a value $m$, $m_s$ denotes a mask which combined with the masked secret $s_m$ would leak the secret $s$. In other words $s = s_{m} \oplus m_{s}$. $m_1$ is a fresh mask independently generated. $p_1$ and $Q$ are public values. Then, the labelling of $G_{1}$, $G_{2}$ and $G_{3}$ are obtained using the rules in Table \ref{tab:rules} for the static (non-glitchy) and transient (glitchy) scenarios as shown in Figure \ref{fig:label_propagation}e and Figure \ref{fig:label_propagation}f respectively. Consider the static case. Figure \ref{fig:label_propagation}b gives the labelling of the gate $G_1$ based on the rules in Table \ref{tab:rules} for the XOR operation. Since for XOR, the labels of the output of the gate is a concatenation of the input labels, hence the result is just a set union of the set of input labels. For the transient case too, this holds for the XOR gate. However for non-linear gates like AND, this does not hold. Consider the gate $G_2$ of the circuit to be verified and its labelling shown in Figure \ref{fig:label_propagation}c. For the static case and the transient case both the output's labels will be a set of all possible combinations of the input sets. This can be drawn from the Fourier expansion of the AND function in Section \ref{subsubsec:rebecca}. Here we can see that for inputs $x$ and $y$ all the possible coefficients in the monomial for $AND(x, y)$: $\{\phi$, $x$, $y$ and $xy\}$, have non-zero values. Given that the output $q$ of the design in Figure \ref{fig:label_propagation}a has been derived correctly in Figure \ref{fig:label_propagation}e. Similarly labels were obtained for the transient case in Figure \ref{fig:label_propagation}f. Given such a labelling REBECCA check each gate output for correlations with secrets. If they do exist, REBECCA further checks if they contain a correlation to a mask unrelated to the secret. If such a mask exists in the correlation set then the gate is secure otherwise it is not secure. 

\begin{figure*}[htbp]
\centering
\begin{minipage}[t]{0.45\textwidth}
\begin{tikzpicture}[node distance=1cm, font=\sffamily, scale=0.6, transform shape]
    % Nodes
    \node (input1) {};
    \node (input2) [below of=input1, yshift=-0.5cm] {};
    \node (input3) [below of=input2, yshift=-0.2cm] {};
    \node (input4) [below of=input3, yshift=-0.5cm] {};
    \node (xor1) [right of=input1, xshift=1.5cm, yshift=-0.5cm, draw, xor gate US, logic gate inputs=nn, anchor=input 1] {XOR};
    \node (and) [right of=input3, xshift=1.5cm, draw, and gate US, logic gate inputs=nn, anchor=input 1] {AND};
    \node (xor2) [right of=and, xshift=0.7cm, yshift=1.4cm, draw, xor gate US, logic gate inputs=nn, anchor=input 1] {XOR};
    \node (output) [right of=xor2, xshift=2cm] {};
   
    % Arrows
    \draw[->] (input1.east) -- ++(0.3,0) |- (xor1.input 1) node[pos=0.75, above] {${S_{m}}$};
    \draw[->] (input2.east) -- ++(0.3,0) |- (xor1.input 2) node[pos=0.75, below] {${m_{1}}$};
    \draw[->] (xor1.output) -- ++(0.3,0) |- (xor2.input 1);
    \draw[->] (input3.east) -- ++(0.3,0) |- (and.input 1) node[pos=0.75, above] {${m_{s}}$};
    \draw[->] (input4.east) -- ++(0.3,0) |- (and.input 2) node[pos=0.75, below] {${p_{1}}$};
    \draw[->] (and.output) -- ++(0.3,0) |- (xor2.input 2);
    \draw[->] (xor2.output) -- (output.west) node[pos=0.35, below] {$q$};
    
    % Labels
    \node [below of=xor1, yshift=-0.5cm] {${G_1}$};
    \node [below of=and, yshift=-0.5cm] {${G_2}$};
    \node [below of=xor2, yshift=-0.5cm] {${G_3}$};
    
    % Caption
    \node [below of=and, yshift=-1cm] {(a) Circuit to be verified};
\end{tikzpicture}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
\begin{tikzpicture}[node distance=1cm, font=\sffamily,scale=0.6, transform shape]
    % Nodes
    \node (input1) [draw, rectangle, text width=1.5cm, align=center] {{$\{ s, m_s \}$}};
    \node (input2) [below of=input1, yshift=-0.5cm, draw, rectangle, text width=1.5cm, align=center] {{$\{ m_1 \}$}};
  
    \node (xor1) [right of=input1, xshift=1.5cm, yshift=-0.5cm, draw, xor gate US, logic gate inputs=nn, anchor=input 1] {XOR};
    
    \node (wire2)[right of=xor1, xshift=1.4cm, draw, rectangle, text width=2.6cm, align=center] {{$\{\{ s,  m_s, m_1\}\}$}};
     
    % Arrows
    \draw[->] (input1.east) -- ++(0.3,0) |- (xor1.input 1)node[pos=0.75, above] {${S_{m}}$};
    \draw[->] (input2.east) -- ++(0.3,0) |- (xor1.input 2)node[pos=0.75, below] {${m_{1}}$};
     \draw[->] (xor1.east) -- ++(0.2,0) |- (wire2);
    % \draw[->] (xor1.output) -- ++(0.3,0) |- (xor2.input 1);
   
    
    % Labels
    % \node [above of=input1, yshift=-0.3cm] {${S_m}$};
    \node [below of=xor1] {${G_1}$};
    
    % \node [right of=output, xshift=1cm] {${q}$};
    
    % Gate label
    \node [below of=xor1, yshift=-1.1cm] {(b) Propagation of labels for the first XOR gate};
\end{tikzpicture}
\end{minipage}
\vspace{1.5cm}
\begin{minipage}[t]{0.45\textwidth}
\begin{tikzpicture}[node distance=1cm, font=\sffamily,scale=0.6, transform shape]
    % Nodes
    
    \node (input3) [below of=input2, yshift=-0.2cm, draw, rectangle, text width=1.5cm, align=center] {{$\{ m_s \}$}};
    \node (input4) [below of=input3, yshift=-0.5cm, draw, rectangle, text width=1.5cm, align=center] {{$\{ p_1 \}$}};
  
    \node (and) [right of=input3, xshift=1.5cm, draw, and gate US, logic gate inputs=nn, anchor=input 1] {AND};
    
  
    \node (wire2)[right of=and, xshift=2.4cm,  draw, rectangle, text width=3.8cm, align=center] {{$\{ \phi,  \{m_s\}, \{ p_1\}, \{ m_s, p_1\}\}$}};
    % Arrows
    
    \draw[->] (input3.east) -- ++(0.3,0) |- (and.input 1)node[pos=0.75, above] {${m_{s}}$};
    \draw[->] (input4.east) -- ++(0.3,0) |- (and.input 2)node[pos=0.75, below] {${p_{1}}$};
    \draw[->] (and.east) -- ++(0.2,0) |- (wire2);
   
    
    % Labels
    % \node [above of=input1, yshift=-0.3cm] {${S_m}$};

    \node [below of=and] {${G_2}$};

    % \node [right of=output, xshift=1cm] {${q}$};
    
    % Gate label
    \node [below of=and, yshift=-1cm] {(c) Propagation of Labels for the AND gate};
\end{tikzpicture}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
\begin{tikzpicture}[node distance=1cm, font=\sffamily,scale=0.6, transform shape]
    % Nodes
   
    \node (xor2) [right of=and, xshift=0.7cm, yshift=1.4cm, draw, xor gate US, logic gate inputs=nn, anchor=input 1] {XOR};
    \node (output) [right of=xor2, xshift=2cm, draw, rectangle, text width=3.2cm, align=center] {{$\{ \{s, m_s, m_1\}, \{s, m_1\}$,\\ $\{s, m_s, m_1, p_1\}, $\\$\{s, m_1, p_1\} \}$}};
    \node (wire2)[right of=xor1,  xshift=-1.7cm, draw, rectangle, text width=2.6cm, align=center] {{$\{\{ s,  m_s, m_1\}\}$}};
    \node (wire2)[right of=and, xshift=-2.4cm, draw, rectangle, text width=3.8cm, align=center] {{$\{ \phi,  \{m_s\}, \{ p_1\}, \{ m_s, p_1\}\}$}};
    % Arrows
   
    \draw[->] (xor1.output) -- ++(0.3,0) |- (xor2.input 1);
    
    \draw[->] (and.output) -- ++(0.3,0) |- (xor2.input 2);
    \draw[->] (xor2.output) -- (output.west)node[pos=0.35, below] {$q$};
    
    % Labels
    % \node [above of=input1, yshift=-0.3cm] {${S_m}$};

    \node [below of=xor2] {${G_3}$};
    % \node [right of=output, xshift=1cm] {${q}$};
    
    % Gate label
    \node [below of=xor2, yshift=-1cm] {(d) Propagation of Labels for the Second XOR gate};
\end{tikzpicture}
\end{minipage}
\vspace{1cm}
\begin{minipage}[t]{0.45\textwidth}
\begin{tikzpicture}[node distance=1cm, font=\sffamily,scale=0.6, transform shape]
    % Nodes
    \node (input1) [draw, rectangle, text width=1.5cm, align=center] {{$\{ s, m_s \}$}};
    \node (input2) [below of=input1, yshift=-0.5cm, draw, rectangle, text width=1.5cm, align=center] {{$\{ m_1 \}$}};
    \node (input3) [below of=input2, yshift=-0.2cm, draw, rectangle, text width=1.5cm, align=center] {{$\{ m_s \}$}};
    \node (input4) [below of=input3, yshift=-0.5cm, draw, rectangle, text width=1.5cm, align=center] {{$\{ p_1 \}$}};
    \node (xor1) [right of=input1, xshift=1.5cm, yshift=-0.5cm, draw, xor gate US, logic gate inputs=nn, anchor=input 1] {XOR};
    \node (and) [right of=input3, xshift=1.5cm, draw, and gate US, logic gate inputs=nn, anchor=input 1] {AND};
    \node (xor2) [right of=and, xshift=0.7cm, yshift=1.4cm, draw, xor gate US, logic gate inputs=nn, anchor=input 1] {XOR};
    \node (output) [right of=xor2, xshift=2cm, draw, rectangle, text width=3.2cm, align=center] {{$\{ \{s, m_s, m_1\}, \{s, m_1\}$,\\ $\{s, m_s, m_1, p_1\}, $\\$\{s, m_1, p_1\} \}$}};
    \node (wire2)[right of=xor1, xshift=1.4cm, yshift=0.5cm, draw, rectangle, text width=2.6cm, align=center] {{$\{\{ s,  m_s, m_1\}\}$}};
     \node (wire2)[right of=and, xshift=1.4cm, yshift=-0.8cm, draw, rectangle, text width=3.8cm, align=center] {{$\{ \phi,  \{m_s\}, \{ p_1\}, \{ m_s, p_1\}\}$}};
    % Arrows
    \draw[->] (input1.east) -- ++(0.3,0) |- (xor1.input 1)node[pos=0.75, above] {${S_{m}}$};
    \draw[->] (input2.east) -- ++(0.3,0) |- (xor1.input 2)node[pos=0.75, below] {${m_{1}}$};
    \draw[->] (xor1.output) -- ++(0.3,0) |- (xor2.input 1);
    \draw[->] (input3.east) -- ++(0.3,0) |- (and.input 1)node[pos=0.75, above] {${m_{s}}$};
    \draw[->] (input4.east) -- ++(0.3,0) |- (and.input 2)node[pos=0.75, below] {${p_{1}}$};
    \draw[->] (and.output) -- ++(0.3,0) |- (xor2.input 2);
    \draw[->] (xor2.output) -- (output.west)node[pos=0.35, below] {$q$};
    
    % Labels
    % \node [above of=input1, yshift=-0.3cm] {${S_m}$};
    \node [below of=xor1] {${G_1}$};
    \node [below of=and] {${G_2}$};
    \node [below of=xor2] {${G_3}$};
    % \node [right of=output, xshift=1cm] {${q}$};
    
    % Gate label
    \node [below of=and, yshift=-1cm] {(e) Using Stable Propagation of Labels};
\end{tikzpicture}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
\begin{tikzpicture}[node distance=1cm, font=\sffamily,scale=0.6, transform shape]
    % Nodes
    \node (input1) [draw, rectangle, text width=1.5cm, align=center] {\textcolor{blue}{$\{ s, m_s \}$}};
    \node (input2) [below of=input1, yshift=-0.5cm, draw, rectangle, text width=1.5cm, align=center] {\textcolor{blue}{$\{ m_1 \}$}};
    \node (input3) [below of=input2, yshift=-0.2cm, draw, rectangle, text width=1.5cm, align=center] {\textcolor{blue}{$\{ m_s \}$}};
    \node (input4) [below of=input3, yshift=-0.5cm, draw, rectangle, text width=1.5cm, align=center] {\textcolor{blue}{$\{ p_1 \}$}};
    \node (xor1) [right of=input1, xshift=1.5cm, yshift=-0.5cm, draw, xor gate US, logic gate inputs=nn, anchor=input 1] {XOR};
    \node (and) [right of=input3, xshift=1.5cm, draw, and gate US, logic gate inputs=nn, anchor=input 1] {AND};
    \node (xor2) [right of=and, xshift=1.7cm, yshift=1.4cm, draw, xor gate US, logic gate inputs=nn, anchor=input 1] {XOR};
    \node (output) [right of=xor2, xshift=2.3cm, draw, rectangle, text width=4.2cm, align=center] {{$\{\textcolor{red}{\{s, m_{s}\}, \textcolor{blue}{\{m_1\},}}$\\$\textcolor{blue}{ \{s, m_s, m_1\}, \{s, m_1\}}$,\\$\textcolor{red}{\{m_s\}, \{ p_1\}, \{ m_s, p_1\}}$\\ $\textcolor{blue}{\{s, m_s, m_1, p_1\}}, \{s\},$\\$\textcolor{red}{\{m_1\}},\textcolor{red}{\{s, m_s, p_1\}, \{ m_1, p_1\},}$\\$\{s, p_1\}, \textcolor{blue}{\{s, m_1, p_1\}} \}$}};
    \node (wire1)[right of=xor1, xshift=1.4cm, yshift=0.7cm, draw, rectangle, text width=2.6cm, align=center] {{$\{\textcolor{red}{\{s, m_{s}\}, \{m_1\},}$\\ $\textcolor{blue}{\{ s,  m_s, m_1\}}\}$}};
    \node (wire2)[right of=and, xshift=1.4cm, yshift=-0.8cm, draw, rectangle, text width=3.8cm, align=center] {\textcolor{blue}{$\{ \phi,  \{m_s\}, \{ p_1\}, \{ m_s, p_1\}\}$}};
    % Arrows
    \draw[->] (input1.east) -- ++(0.3,0) |- (xor1.input 1)node[pos=0.75, above] {${S_{m}}$};
    \draw[->] (input2.east) -- ++(0.3,0) |- (xor1.input 2)node[pos=0.75, below] {${m_{1}}$};
    \draw[->] (xor1.output) -- ++(0.3,0) |- (xor2.input 1);
    \draw[->] (input3.east) -- ++(0.3,0) |- (and.input 1)node[pos=0.75, above] {${m_{s}}$};
    \draw[->] (input4.east) -- ++(0.3,0) |- (and.input 2)node[pos=0.75, below] {${p_{1}}$};
    \draw[->] (and.output) -- ++(0.3,0) |- (xor2.input 2);
    \draw[->] (xor2.output) -- (output.west)node[pos=0.35, below] {$q$};
    
    % Labels
    % \node [above of=input1, yshift=-0.3cm] {${S_m}$};
    \node [below of=xor1] {${G_1}$};
    \node [below of=and] {${G_2}$};
    \node [below of=xor2] {${G_3}$};
    % \node [right of=output, xshift=1cm] {${q}$};
    
    % Gate label
    \node [below of=and, yshift=-1cm] {(f) Using Transient Propagation of Labels};
\end{tikzpicture}
\end{minipage}
\caption{Label propagation through logic gates in the verification circuit.}
\label{fig:label_propagation}
\end{figure*}
\begin{table}[H]
    \centering
    \vspace{3mm}
    \caption{Initial labelling for the design in Example given in Figure \ref{fig:label_propagation}}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{|c|c|c|c|}
        \hline
        \textbf{No.} & \textbf{Inputs} & \textbf{Label} & \textbf{Correlation set} \\
        \hline
        1 & $s_m$ & Share 1 & \{ $s_1$, $m_2$ \} \\
        \hline
        2 & $m_s$ & Share 1 & \{ $m_2$ \} \\
        \hline
        3 & $m_1$ & Mask & \{ $m_1$ \} \\
        \hline
        4 & $p_1$ & Unimportant (public value) & \{ $y_1$ \} \\
        \hline
        5 & $q$ & Unimportant (public value) & \{ $y_2$ \} \\
        \hline
        6 & XOR ($G_1$) & - & - \\
        \hline
        7 & AND ($G_2$) & - & - \\
        \hline
        8 & XOR ($G_3$) & - & - \\
        \hline
    \end{tabular}%
    }
    \label{tab:example}
\end{table}


\begin{table}[H]
\small % Reduce font size
\setlength{\tabcolsep}{3pt} % Reduce column padding
\renewcommand{\arraystretch}{1.1} % Slightly more row padding for readability
\centering
\caption{Rules for Gates, Stable, and Transient States}
\begin{tabular}{|c|c|c|c|}
\hline
& \textbf{Gates} & \textbf{Stable} & \textbf{Transient} \\
\hline
Wire & 
\begin{tikzpicture}[scale=0.7]
    \draw (0,0) node[left] {$a$} -- (1,0) node[right] {$a$};
\end{tikzpicture} & 
$\{a\}$ & $\{a\}$ \\
\hline
NOT & 
\begin{tikzpicture}[circuit logic US, scale=0.6]
    \node[not gate, draw, logic gate inputs=none] (NOT1) at (0,0) {};
    \draw (NOT1.input) -- ++(-0.4,0) node[left] {$a$};
    \draw (NOT1.output) -- ++(0.4,0) node[right] {$a^\prime$};
\end{tikzpicture} & 
$\{a\}$ & $\{a\}$ \\
\hline
AND/NAND & 
\begin{tikzpicture}[circuit logic US, scale=0.6]
    \node[and gate, draw, logic gate inputs=nn] (AND1) at (0,0) {};
    \draw (AND1.input 1) -- ++(-0.4,0) node[left] {$a$};
    \draw (AND1.input 2) -- ++(-0.4,0) node[left] {$b$};
    \draw (AND1.output) -- ++(0.4,0) node[right] {$c$};
\end{tikzpicture} & 
$S_a \otimes S_b$ & $T_a \otimes T_b$ \\
\hline
Register & 
\begin{tikzpicture}[scale=0.6]
    \draw (0,0) node[left] {$a$} -- (0.4,0);
    \draw (0.4,0.25) rectangle (1,-0.25);
    \draw (1,0) -- (1.4,0) node[right] {$a$};
\end{tikzpicture} & 
$\{a\}$ & $\{a\}$ \\
\hline
XOR/XNOR & 
\begin{tikzpicture}[circuit logic US, scale=0.6]
    \node[xor gate, draw, logic gate inputs=nn] (XOR1) at (0,0) {};
    \draw (XOR1.input 1) -- ++(-0.4,0) node[left] {$a$};
    \draw (XOR1.input 2) -- ++(-0.4,0) node[left] {$b$};
    \draw (XOR1.output) -- ++(0.4,0) node[right] {$c$};
\end{tikzpicture} & 
$S_a \oplus S_b$ & $T_a \oplus T_b$ \\
\hline
MUX & 
\begin{tikzpicture}[scale=0.5]
    \draw (0,1) -- (1,0.8) -- (1,-0.8) -- (0,-1) -- cycle;
    \draw (-0.8,0.5) node[left] {$a$} -- (0,0.5);
    \draw (-0.8,-0.5) node[left] {$b$} -- (0,-0.5);
    \draw (1,0) -- (1.8,0) node[right] {$y$};
    \draw (0.5,-1) -- (0.5,-1.2) -- (-0.8,-1.2) node[left] {$c$};
    \node at (0.5,0) {\footnotesize MUX};
\end{tikzpicture} & 
$S_c \otimes (S_a \cup S_b)$ & $T_a \otimes T_b \otimes T_c$ \\
\hline
\end{tabular}

\label{tab:rules}
\end{table}



